Lean Census: A Distributional Analysis of AI-Generated Lean Code

We compare two human-written and four AI-generated Lean libraries with Mathlib through the distributions of simple statistics of their code. For each library we measure inline claims in proofs, proof length, how often each declaration is used, and design choices such as instances and private declarations, and we read each against the variation among Mathlib's own areas. The AI-generated libraries have more inline claims per theorem, longer proofs, fewer instances, and more private declarations than the human-written ones. We release the code for the analysis as a package, lean-census, at https://github.com/project-numina/lean-census.

==> generated/headline.tex <==
Mathlib & 0.21 & 10\% & 31\% & 10.7\% & 1.1\% & 23\% \\
\rowrule
Mathlib areas & 0.03--0.52 & 2--23\% & & 2.2--27.4\% & 0.0--6.9\% & 7--37\% \\
\rowrule
CSLib & 0.31 & 15\% & 36\% & 6.2\% & 4.1\% & 24\% \\
\rowrule
PhysLib & 0.64 & 21\% & 43\% & 5.4\% & 3.4\% & 31\% \\
\rowrule
FormalFrontier & 0.81 & 25\% & 37\% & 2.7\% & 17.2\% & 54\% \\
\rowrule
Tau Ceti & 0.89 & 30\% & 42\% & 3.2\% & 14.0\% & 44\% \\
\rowrule
CSLib Frontier & 1.61 & 37\% & 51\% & 0.8\% & 18.7\% & 44\% \\
\rowrule
Atlas & 3.22 & 49\% & 61\% & 1.2\% & 37.1\% & 47\% \\


==> generated/inventory.tex <==
\multicolumn{10}{@{}l}{\textbf{Reuse as compression}} \\
\quad Reuse score, weighted by length & 7.9$\times$ & 2.1$\times$--21.1$\times$ & 7.1$\times$ & 5.3$\times$ & 3.1$\times$ & 4.3$\times$ & 4.2$\times$ & 2.2$\times$ & +0.61 \\
\quad Reuse score, weighted by statement length & 6.4$\times$ & 2.2$\times$--13.6$\times$ & 7.3$\times$ & 5.0$\times$ & 2.7$\times$ & 4.1$\times$ & 4.6$\times$ & 2.6$\times$ & +0.62 \\
\quad Reuse score, unweighted & 9.7$\times$ & 2.9$\times$--17.9$\times$ & 8.7$\times$ & 8.9$\times$ & 4.2$\times$ & 7.3$\times$ & 9.0$\times$ & 4.3$\times$ & +0.65 \\
\quad Reuse score, uses from other files & 5.6$\times$ & 1.2$\times$--16.0$\times$ & 2.5$\times$ & 3.6$\times$ & 1.7$\times$ & 2.7$\times$ & 2.8$\times$ & 1.3$\times$ & +0.69 \\
\quad Instances among declarations & 10.7\% & 2.2\%--27.4\% & 6.2\% & 5.4\% & 2.7\% & 3.2\% & 0.8\% & 1.2\% & -0.18 \\
\quad Local helpers & 37\% & 32\%--51\% & 38\% & 39\% & 47\% & 39\% & 50\% & 71\% & -0.60 \\
\quad Single-use theorems & 29\% & 21\%--46\% & 37\% & 39\% & 34\% & 35\% & 46\% & 53\% & -0.33 \\
\quad References that leave the file & 71\% & 17\%--78\% & 55\% & 70\% & 41\% & 65\% & 65\% & 34\% & +0.79 \\
\quad Used from another file & 29\% & 12\%--38\% & 30\% & 39\% & 22\% & 42\% & 38\% & 14\% & +0.40 \\
\quad References to the top 1\% & 57\% & 10\%--67\% & 31\% & 40\% & 28\% & 40\% & 40\% & 28\% & +0.83 \\
\addlinespace
\multicolumn{10}{@{}l}{\textbf{Lemmas that were not factored out}} \\
\quad Inline claims per theorem (have, suffices) & 0.21 & 0.03--0.52 & 0.31 & 0.64 & 0.81 & 0.89 & 1.61 & 3.22 & -0.20 \\
\quad Theorems with an inline claim & 10\% & 2\%--23\% & 15\% & 21\% & 25\% & 30\% & 37\% & 49\% & -0.23 \\
\quad Inline claims per used theorem & 0.28 & 0.05--0.61 & 0.37 & 0.76 & 1.06 & 1.00 & 1.79 & 3.47 & -0.08 \\
\quad Inline claims per unused theorem & 0.09 & 0.02--0.52 & 0.20 & 0.31 & 0.41 & 0.46 & 0.63 & 2.17 & -0.48 \\
\quad Destructuring steps per theorem & 0.18 & 0.06--0.41 & 0.41 & 0.21 & 0.30 & 0.34 & 0.64 & 0.69 & -0.01 \\
\quad Explicit unfoldings per theorem & 0.01 & 0.00--0.04 & 0.01 & 0.03 & 0.01 & 0.01 & 0.10 & 0.14 & -0.40 \\
\quad Inline claims including obtain & 0.27 & 0.04--0.62 & 0.50 & 0.75 & 0.98 & 1.09 & 1.89 & 3.55 & -0.19 \\
\quad Proof text in proofs over 200 tokens & 26\% & 0\%--53\% & 23\% & 51\% & 54\% & 45\% & 62\% & 74\% & -0.16 \\
\quad Proof text in the longest 1\% of proofs & 18\% & 7\%--23\% & 13\% & 20\% & 15\% & 10\% & 15\% & 18\% & +0.42 \\
\addlinespace
\multicolumn{10}{@{}l}{\textbf{Proof information}} \\
\quad Compressed proof per theorem (bits) & 338 & 166--528 & 305 & 561 & 654 & 697 & 903 & 1176 & -0.16 \\
\quad Compressed proof per compressed statement & 1.0 & 0.8--2.1 & 1.2 & 1.7 & 1.3 & 1.3 & 1.6 & 2.2 & -0.55 \\
\quad Bits per proof token & 12.3 & 8.7--11.8 & 9.3 & 8.6 & 9.1 & 11.3 & 9.0 & 7.3 & +0.86 \\
\addlinespace
\multicolumn{10}{@{}l}{\textbf{Source redundancy}} \\
\quad Bits per token & 9.9 & 6.5--9.0 & 7.4 & 7.8 & 7.8 & 9.7 & 8.4 & 7.3 & +0.73 \\
\quad Bits per token given Mathlib & 8.0 & 6.1--8.2 & 7.0 & 7.3 & 7.1 & 8.8 & 8.0 & 6.8 & +0.70 \\
\quad Repeated proof text & 0\% & 1\%--13\% & 8\% & 6\% & 2\% & 0\% & 1\% & 1\% & -0.82 \\
\addlinespace
\multicolumn{10}{@{}l}{\textbf{Distance from Mathlib's idiom}} \\
\quad Trigram bits under a Mathlib model & 6.9 & 7.1--8.7 & 9.8 & 8.8 & 7.9 & 8.1 & 9.4 & 8.3 & -0.47 \\
\quad Information not predictable from Mathlib & 80\% & 89\%--95\% & 95\% & 93\% & 91\% & 90\% & 95\% & 92\% & -0.52 \\
\addlinespace
\multicolumn{10}{@{}l}{\textbf{Other ideas tried}} \\
\quad Theorem leverage inside the library (log2) & 10.0 & 2.4--29.2 & 4.6 & 7.3 & 4.2 & 5.5 & 4.8 & 2.5 & +0.47 \\
\quad Theorems about a definition (median) & 2 & 0--15 & 2 & 3 & 3 & 5 & 3 & 2 & -0.38 \\
\quad Definitions with under 3 theorems & 57\% & 0\%--87\% & 54\% & 43\% & 41\% & 30\% & 40\% & 54\% & +0.22 \\
\quad Theorems stated twice & 2\% & 0\%--9\% & 0\% & 1\% & 1\% & 1\% & 1\% & 2\% & -0.09 \\
\quad Ad hoc names & 1\% & 0\%--4\% & 2\% & 2\% & 0\% & 1\% & 2\% & 4\% & -0.07 \\
\addlinespace
\multicolumn{10}{@{}l}{\textbf{Elaborated terms}} \\
\quad Sharing inside proof terms & 4.4$\times$ & 1.7$\times$--37.6$\times$ & 2.5$\times$ & 21.0$\times$ & 16.1$\times$ & 22.4$\times$ & 7.9$\times$ & 10.4$\times$ & -0.19 \\
\quad Proof term nodes per proof token & 22.1 & 11.0--97.7 & 12.6 & 27.7 & 21.9 & 26.5 & 11.7 & 11.2 & -0.05 \\
\quad Unwrapped length per token (log2) & 73 & 16--229 & 42 & 201 & 115 & 166 & 74 & 95 & -0.19 \\


==> generated/tables.tex <==
CSLib & 1.65 & 1.91 & 1.43 & 1.47 \\
\rowrule
PhysLib & 1.69 & 1.53 & 1.16 & 1.46 \\
\rowrule
FormalFrontier & 1.48 & 2.92 & 1.37 & 1.21 \\
\rowrule
Tau Ceti & 0.79 & 2.94 & 1.31 & 1.44 \\
\rowrule
CSLib Frontier & 1.67 & 3.01 & 1.19 & 0.62 \\
\rowrule
Atlas & 1.75 & 3.22 & 1.65 & 0.68 \\

